LASER: Linear Compression in Wireless Distributed Optimization

Data-parallel SGD is the de facto algorithm for distributed optimization, especially for large scale machine learning. Despite its merits, communication bottleneck is one of its persistent issues. Most compression schemes to alleviate this either assume noiseless communication links, or fail to achieve good performance on practical tasks. In this paper, we close this gap and introduce LASER: LineAr CompreSsion in WirEless DistRibuted Optimization. LASER capitalizes on the inherent low-rank structure of gradients and transmits them efficiently over the noisy channels. Whilst enjoying theoretical guarantees similar to those of the classical SGD, LASER shows consistent gains over baselines on a variety of practical benchmarks. In particular, it outperforms the state-of-the-art compression schemes on challenging computer vision and GPT language modeling tasks. On the latter, we obtain $50$-$64 \%$ improvement in perplexity over our baselines for noisy channels.

==> comprx_accuracy.tex <==
% !TEX root = main.tex

\subsection{Compression rate and accuracy}
\label{sec:cmpx_power}

It is important to note that the interplay between compression and accuracy is deeply influenced by the presence of noise in the transmission in our model. This is due to the power constraint that we impose in \prettyref{eq:normal_awgn}. In fact, if the gradient communication is noiseless, which is equivalent to assume that infinite power is available for the transmission, one expects that a higher compression of the gradients implies worse final accuracy, and that the best performance is achieved by sending the full uncompressed gradients to the server. This is no longer true if some power constraint is imposed to the users. In such a setting, sending compressed gradients -- i.e., sending fewer numbers -- means that one can use more power per entry, and as a result, the transmitted data will be less corrupted by noise. Therefore, sending the largest amount of information with the smallest amount of data becomes critical. It is then clear that the relation between compression factor and final accuracy is not obvious anymore in this context, and one may even achieve higher accuracy by sending compressed gradients with respect to sending the full uncompressed data, which would be more heavily corrupted by noise due to the limited power available. Therefore, to better understand the interplay of compression and accuracy, further experimental analysis is required, in order to determine which algorithm, for a fixed compression factor -- i.e., fixed amount of transmitted data -- is able to pack and send the largest amount of information about the gradients.

We investigate this relationship in \prettyref{fig:cf-accuracy}, where we tested the different algorithms in two power regimes: low ($P=?$) and medium power ($P=?$). For each power regime, we computed the final test accuracy for each algorithm, for several compression factors. It is worth pointing out that for \textsc{Random-K}, \textsc{Top-K}, \textsc{Count-Mean Sketching} and \textsc{A-DSGD}, essentially any fraction between 0 and 1 is a valid compression factor choice, since these methods rely either on preserving only a selected percentage of entries of the gradients, or they project gradients on a chosen lower-dimensional space. In \textsc{LASER}, the choice of the compression factor is more restricted, since it is a direct consequence of the chosen approximation rank. As a rule, we first selected several rank values for LASER. Then, we computed the effective compression factor for each rank choice, by dividing the number of entries \emph{after} compression by the total number of uncompressed parameters. Then, the resulting compression factor is imposed to the other algorithms. For \textsc{LASER}, the same rank compression is chosen for all the gradients in the network. Similarly, the same compression factor is fixed for all gradients when testing the other baselines.










==> exp_setup.tex <==
% !TEX root = main.tex

{\bf Setup.} We consider three challenging tasks of practical interest: (i) image classification on \cifarten and \cifarhun , and (ii) language modeling on \wikileaks. For the classification task, we use the standard \resnet architecture, widely adopted in the literature. For the language modeling, we use the \nanogpt implementation of \nb{}. For distributed training of these models, we consider $k=16$ workers. We simulate the noisy channel by sampling $\bZ \sim \calN(0, \id_d)$. We vary the power level $P$ over $\{\ldots \}$ to gauge the performance of algorithms over a wide range of noisy conditions. This range can be roughly split into low-moderate-high power regimes. Recall from \ref{eq:awgn_final} that smaller the power, higher the noise in the channel and vice-versa. 

{\bf Baselines.} We compare \miss with three different sets of baselines: (i) SignSGD, Top-K, Rand-K, Count-Mean-Sketching, (ii) A-DSGD, (iii) Z-SGD. The algorithms in (i) are competitive gradient compression schemes primarily designed for noiseless distributed communication. Our goal here is to check how robust these methods are to communication noise. A-DSGD is a popular state-of-the-art gradient compression scheme for noisy channels, which relies on Top-K and random sketching ideas. However, A-DSGD is memory intensive and is only limited to MNIST classification and doesn't scale to either of the three tasks of interest. Hence for a fair comparison, we compare \miss with A-DSGD on MNIST too. \ref{eq:awgn_sgd} sends the uncompressed gradients directly over the noisy channel. We also compare with the noiseless \ref{eq:sgd}. At each power $P$, we consider the best compression factor for each of the baselines in the range $[0.1, 0.8]$.






%\subsection{Experimental setup}
%We now describe in more detail our experimental setup, in particular the tasks and the methods we compared to.
%
%\paragraph{Benchmarks}
%We tested LASER on three tasks, in order to show the broad applicability of our method. For image classification tasks, we used the standard CIFAR-10 and CIFAR-100 datasets, both learned using a ResNet-18 model. For language prediction, instead, we used \textsc{WikiText} and a \textsc{LLM} architecture inspired by \textsc{NanoGPT} \cite{}. See Table \ref{tab:tasks} for a summary of the tasks.
%
%\paragraph{Baselines}
%We compared \textsc{LASER} against a wide selection of algorithms, comprising methods designed for gradient compression in both noiseless and noisy case. In the first category fall \textsc{Random-K}, \textsc{Top-K}, and \textsc{Count-Mean Sketching}. These algorithms originally assume that the communication between the clients and the server is noiseless; therefore, we study the effect of noise on their performance. In the second category falls \textsc{A-DSGD}, which is designed for noisy wireless communication over an additive channel, which is the same setting as ours. In the original paper, the algorithm is tested in the case of a simple single-layer neural network for a image classification task on the \textsc{MNIST} datatset. In this paper, we study its scalability by applying it to the more complex tasks of image classification on \textsc{Cifar-10} and \textsc{Cifar-100}, as well as on text prediction on \textsc{WikiText}. Finally, we compare the baselines to the uncompressed case, i.e., to sending the full gradients through the noisy channel without any compression; we refer to this approach by \textsc{Z-SGD}.
%
%Each algorithm is implemented with local \emph{error feedback}. The algorithms' description can be found in Appendix. The code for each algorithm is publicly available, with the exception of \textsc{A-DSGD}, which was implemented following private correspondence with the authors.
%
%\paragraph{Tuning of parameters}
%In our setting, we can divide the set of tunable parameters into two categories: the neural network hyper-parameters, which exclusively affect the local neural network training, and the communication parameters, which affect the (noisy) communication between the clients and the server. Regarding the neural network hyper-parameters, we fixed the number of epochs/iterations and the batch size, and we studied the interplay between learning rate and power on the final accuracy. In particular, we noticed that a low learning rate is more suitable in the low-power regime, while a higher one works better in the high-power regime. The same behavior was observed for all the considered algorithms.
%
%The communication parameters, instead, include the number of workers, the compression factor, the power constraint $P$, which, due to \prettyref{eq:awgn_final}, determines the effective noise level of the communication channel, and the power allocation. To highlight the general validity of our method, we run the experiments both in the single-worker case, and in the case of 16 workers. Since in this work we are not interested in the actual clock times taken by the algorithms (for the time savings of PowerSGD compared to other compression methods, we refer to \cite{vogels2019powersgd}), the multiple-worker case is simulated code-wise, and the experiments are run on a single machine. For each algorithm, several compression factors were considered; further details can be found in \prettyref{sec:cf-accuracy}, where we discuss how the amount of compression influences the final test accuracy of the model. Furthermore, we analyzed a wide range of power constraints, which can be roughly divided in the three regimes: \emph{low power, medium power} and \emph{high power}.
%
%The final, and perhaps most important, tuning aspect is power allocation. Notice that, because of \prettyref{eq:weightedgrad_awgn}, all clients must allocate the same power to a given gradient, since otherwise it would be impossible to recover the correct average gradient. However, workers have a degree of freedom in choosing how to distribute the power budget among gradients, i.e., among the layers of the network, and this power allocation can change over the iterations of the model training. In this work, we considered the following power allocation scheme: at each iteration, each worker determines locally how to allocate its power budget across the gradients. Then, we assume that this power allocation choice is communicated by the client to the server noiselessly. The server then takes the average of the power allocation choices, and communicates the final power allocation to the clients. The clients then use this power allocation to send the gradients to the server via the noisy channel. For the determination of each worker's power allocation, several schemes were considered: uniform power to each gradient, power proportional to the number of entries in each gradient, power proportional to the Frobenius norm (or the square of it) of the gradients, and finally, power proportional to the norm of the compressed gradients (i.e., the norm of what is actually communicated to the server). For \textsc{Z-SGD}, where there is no gradient compression, the best power allocation turned out to be the one proportional to the norm of the gradients, independently of the power constraint imposed. For all the other algorithms, the best is power proportional to the norm of the compressed gradients.


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> problem_formulation.tex <==
% !TEX root = main.tex

\section{Background}
\label{sec:background}


{\bf Distributed optimization}. Consider the (synchronous) data-parallel distributed setting where we minimize an objective $f:\reals^d \to \reals $ defined as the empirical loss on a global dataset $\calD=\{(\bx_j, y_j)\}_{j=1}^N $: 
\looseness=-1
\begin{align*}
\min_{\btheta \in \reals^d} f(\btheta), \quad f(\btheta) \define \frac{1}{N} \sum_{j=1}^N \ell(\bx_j, y_j ;\btheta),
\end{align*}
where $\ell(\cdot)$ evaluates the loss for each data sample. In this setup, there are $k$ training clients, where the $i$-th client has access to a stochastic gradient oracle $\bg_i$, e.g., mini-batch gradient on a set of samples randomly chosen from $\calD$, such that $\Expect[\bg_i|\btheta] = \nabla f(\btheta)$ for all $\btheta \in \reals^d$. 
%In this setup, there are $k$ training nodes/workers/clients that have each access to a stochastic gradient oracle $\bg$ such that $\Expect[\bg|\btheta] = \nabla f(\btheta)$ for all $\btheta \in \reals^d$. For instance, $\bg$ could be the mini-batch gradient on a set of samples randomly chosen from $\calD$. 
In this context, distributed SGD \cite{robbins1951stochastic, bottou2018optimization} performs the following updates:
\begin{align}
   \btheta_{t+1} = \btheta_t -  \gamma_t \cdot \frac{1}{k} \sum_{i=1}^k \bg_i^{(t)}, \quad \Expect[\bg_i^{(t)}|\btheta_t] = \nabla f(\btheta_t), \quad t \geq 0.
  \label{eq:sgd}
  \tag{SGD}
\end{align}
where $\{\gamma_t \}_{t \geq 0}$ is a step-size schedule. Implicit here is the assumption that the communication link between the clients and the server is noiseless, which we expound upon next.

% Underpinning the above SGD updates is the assumption that the central server receives the local gradients exactly, which maynot always hold as discussed in \prettyref{sec:intro}. We now introduce a canonical communication framework betwen the clients and the server below. 



% samples is split across $k$ distributed workers/clients with $\calD = \cup_{i \in [k]} \calD_i$. The local dataset $\calD_i =\{(\bx_j, y_j)\}_{j=1}^{n_i} $ is of size $n_i = N/k$ (for simplicity). The objective here is to minimize a function $f: \reals^d \to \reals$ in a distributed fashion as follows:

% where $f(\cdot)$ is defined as the average of the local loss functions $\ell_i(\cdot)$ over all the $k$ clients and $\ell_i$ is given by the empirical loss on the local dataset $\calD_i $ for a suitable loss function $\ell(\cdot)$. 


% We assume that there is a global central server that houses the parameter $\btheta$ and that all the clients share the same $\btheta$. Here we focus on the stochastic gradient setup where each worker has access to a stochastic gradient oracle $\bg_i$ of $f$ such that $\Expect[\bg_i] = \nabla f$. At every training iteration, all the clients communicate their local (stochastic) gradients $\{\bg_i\}$ to the central server to update the model parameters $\btheta$. \nb{} illustrates this setup. An important aspect of this distributed framework is the communication channel betwen the clients and the server which we explain below.


{\bf Communication model.} We consider the additive noise (AN) channels to model the communication uplink from the clients to the server. We denote the channel as a (random) mapping $\awgn_P(\cdot)$, that transforms the set of messages transmitted by the clients $\{\bx_i \}_{ i \in [k]} \subset \reals^d $ to its noisy version $\by \in \reals^d$ received by the server:
\looseness=-1
\begin{align}
     \label{eq:normal_awgn}
    \by = \awgn_P(\setx) \define \sum_{i=1}^k \bx_i + \bZ, \quad \norm{\bx_i}^2 \leq P,
\end{align}
where the power $P >0 $ is fixed and known to everyone. The defining property of this family is the superposition of incoming wireless signals (enabling over-the-air computation) possibly corrupted together with an independent channel noise \cite{shi2020communication}. This class comprises some of the well-studied practical channels including the classical multiple-access-channel \cite{nazer2007computation}. 


{\bf {\em Power}} The power constraint indirectly serves as a communication cost and encourages compression: if each client can transmit the same information $\bx_i$ via fewer entries, they can utilize more power per entry and hence a more faithful signal. We assume that the noise $\bZ \in \reals^d$ is independent of the channel inputs and has zero mean and unit variance per dimension. 
A key metric that captures the channel degradation quality is the signal-to-noise ratio per coordinate ($\snr$), defined as $\snr \define P/d $ (for signals of size $m\times n$, $\snr \define P/mn$). The larger it is the better the signal fidelity; $\snr = \infty$ corresponds to the ideal scenario when there is no noise. For the downlink communication from the server to the clients (broadcast channel), we assume that it is noiseless and thus the clients receive exactly what the server transmits \cite{fedoriginal17, fedefficiency16, fedoptim16}. In the rest of the paper by channel we mean the uplink channel. 

{\bf Gradient transmission over the channel.} In the distributed optimization setting the goal is to communicate the local gradients $\bg_i \in \reals^d$ to the central server over the noisy channel in \prettyref{eq:normal_awgn}. Here we set the messages $\bx_i$ as linear scaling of gradients (given the linear channel), \ie $\bx_i = a_i \, \bg_i$ with the scalars $a_i \in \reals$ enforcing the power constraints:
\begin{align}
    \label{eq:weightedgrad_awgn}
    \by  =  \sum_{i=1}^k a_i \, \bg_i + \bZ, \quad \norm{a_i \, \bg_i}^2 \leq P.
\end{align}
Now the received signal is a weighted summation of the gradients corrupted by noise, whereas we need the sum of the gradients $\sum_i \bg_i$ (up to zero mean additive noise) for the model training. Towards this goal, a common mild technical assumption is that the gradient norms $\{ \norm{\bg_i} \}$ are known at the receiver at each communication round
\cite{chang2020mac, guo2020analog} (can be relaxed in practice, \prettyref{sec:main_results}). The optimal scalars are then given by $a_i  =\sqrt{P}/(\max_j \norm{\bg_j}), \forall i \in [K]$, which are uniform across all the clients (\S~\ref{app:channel_transf}). 
% In other words, during each communication round the clients transmit their gradient norms to the server which then computes their maximum and broadcasts it back to them to compute $a_i$. 
Now substituting this $a_i$ in \prettyref{eq:weightedgrad_awgn} and rearranging, the effective channel can be written as
\begin{align}
    \by = \tilde{\awgn}_{P}(\setg) \define \frac{1}{k} \sum_{i=1}^k \bg_i + \frac{\max_i \norm{\bg_i}}{k \sqrt{P}} \, \bZ.
    \tag{noisy channel}
    \label{eq:awgn_final}
\end{align}
Or equivalently, we can assume this as the actual channel model where the server receives the gradient average corrupted by a zero mean noise proportional to the gradients. Note that the noise magnitude decays in time as gradients converge to zero.
% When there is just a single worker, $k=1$, this simplifies to
% \begin{align}
%     \label{eq:awgn_single}
%     \by = \awgn_{P, \mathrm{eff}}(\bg_1) = \bg_1 + \frac{\norm{\bg_1}}{\sqrt{P}} \, \bZ.
% \end{align}
We denote $\tilde{\awgn}_{P}(\cdot)$ as simply $\awgn_P(\cdot)$ henceforth as these two mappings are equivalent.

%%%%
% Removed for brevity
%%%%
% Hence the scalars $a_i$ have to be chosen properly so as to meet the following two objecives: (i) enforcing the power constraint $P$ on gradients, and (ii) ensuring an unbiased estimate of the gradient sum at the receiver. 

{\bf Z-SGD.} In the presence of the noisy channel, the \ref{eq:sgd} algorithm modifies to
\begin{align}
\btheta_{t+1} = \btheta_t - \gamma_t \, \awgnp(\{\bg_i^{(t)} \} ).
    \tag{Z-SGD}
    \label{eq:awgn_sgd}
\end{align}
Note that the Z-SGD has two sources of stochasticity: one stemming from the stochastic gradients and the other from the channel noise. While the gradient used in the Z-SGD update still has the same conditional mean as the noiseless case  (zero mean Gaussian in ~\ref{eq:awgn_final}), it has higher variance due to the Gaussian term. When $P = \infty$, \ref{eq:awgn_sgd} reduces to \ref{eq:sgd}. 


% For training the model parameters $\btheta$ at the client using the (synchronous) distributed SGD algorithm, we follow the following communication protocol at each iteration $t$: (i) all the clients compute the local gradients $\bg_i$ based on $\btheta_t$ and transmit their norms $\norm{\bg_i}$ to the client; (ii) the server transmits them back the maximum of these norms $\max_i \norm{\bg_i}$; (iii) the clients transmit $\bx_i = \sqrt{P}/(\max_j \norm{\bg_j}) \cdot \bg_i $ and the server receives $\by = \sum_i \sqrt{P}/(\max_j \norm{\bg_j}) \cdot \bg_i + \calN(0,I_d) $; (iv) the server does a simple rescaling to obtain $\by$ as in \prettyref{eq:awgn_final}: $\by = \awgn(\setg) = \sum_i \bg_i + \max_j \norm{\bg_j}/\sqrt{P} \cdot \calN(0,I_d) $; (v) serves uses $\by$ to update the parameters to $\btheta_{t+1}$ which it broadcasts to all the clients. These steps (i)-(v) are again repeated at $t+1$ and so forth. We term this algorithm {\it AWGN-SGD}.

==> results_analysis.tex <==
% !TEX root = main.tex

{\bf Results.} On \cifarten, \prettyref{fig:cifar10} highlights that \miss outperforms the baselines on a wide range of power levels. In particular, we observe that \miss achieves accuracy gains of \nb{x} in the low-power regime and \nb{y} in the moderate region. In the high-power regime, all the baselines are close to the 	SGD baseline as the channel is almost noiseless. \nb{Figure 1b} further illustrates that for the same target accuracy, \miss requires just $(1/8)^{\text{th}}$ power compared to the baselines in the low-regime and a factor of $1/4$ in the moderate regime. We observe similar gains for \cifarhun, which we defer to \nb{}.

Similarly for \nanogpt on \wikileaks, \prettyref{fig:wiki} demonstrates similar gains over the baselines on a wide range of power levels in $\{\ldots\}$: achieving accuracy gains of \nb{x} in the low-regime and \nb{y} in the moderate. Fraction of power.

%\subsection{Interplay between power and accuracy}
%\label{sec:power-accuracy}
%
%As a general quality metric for the algorithms, we chose to use the final test accuracy after a fixed number of epochs for a given power constraint. For the power constraint levels, we considered the values $P \in \{250, 500, 1000, 2000, 4000, 8000, 16000, 32000, 64000, 128000\}$ for the image classification tasks, and $P\in\{\}$ for the language prediction task. For the image classification tasks, at $P = 128000$, all compression methods achieve roughly the same final accuracy, which also coincides with the noiseless uncompressed baseline. Thus, we can consider power levels higher than that as basically equivalent to the noiseless case. For each algorithm, we tried several learning rates in the range $[0.0001 - 0.1]$ and selected the best one for each power constraint. Similarly, we selected the best compression factor among a few in the range $[0.1 - 0.8]$. The number of epochs and the batch size were fixed respectively at $100$ and $1024$ for the single worker case, and at $150$ and $128$ for the 16-workers case. As pointed out above, several power allocation schemes were tried for each algorithm, and the best (power proportional to the norm of the compressed gradients) was selected. The final results of these experiments are shown in \prettyref{fig:} for the language model task, and in \prettyref{fig:} for the image classification task on \textsc{Cifar-10}. From this analysis, \textsc{LASER} is shown to outperform the other methods is roughly every power level, achieving a significantly higher final accuracy then the other methods for any fixed power budget. Furthermore, \textsc{LASER} manages to achieve the same final accuracy then the other algorithms using between 4 and 10 times less power.


==> temp_problem_formulation.tex <==
% !TEX root = main.tex

\section{Background}
\label{sec:background}


{\bf Distributed optimization}. Consider the (synchronous) data-parallel distributed setting where we minimize an objective $f:\reals^d \to \reals $ defined as the empirical loss on a global dataset $\calD=\{(\bx_j, y_j)\}_{j=1}^N $: 
\looseness=-1
\begin{align*}
\min_{\btheta \in \reals^d} f(\btheta), \quad f(\btheta) \define \frac{1}{N} \sum_{j=1}^N \ell(\bx_j, y_j ;\btheta),
\end{align*}
where $\ell(\cdot)$ evaluates the loss for each data sample. In this setup, there are $k$ training \clients, where each $i$-th \client\ has access to a stochastic gradient oracle $\bg_i$, e.g., mini-batch gradient on a set of samples randomly chosen from $\calD$, such that $\Expect[\bg_i|\btheta] = \nabla f(\btheta)$ for all $\btheta \in \reals^d$. 
%In this setup, there are $k$ training nodes/workers/clients that have each access to a stochastic gradient oracle $\bg$ such that $\Expect[\bg|\btheta] = \nabla f(\btheta)$ for all $\btheta \in \reals^d$. For instance, $\bg$ could be the mini-batch gradient on a set of samples randomly chosen from $\calD$. 
In this context, distributed SGD \cite{robbins1951stochastic, bottou2018optimization} performs the following updates:
\begin{align}
   \btheta_{t+1} = \btheta_t -  \gamma_t \cdot \frac{1}{k} \sum_{i=1}^k \bg_i^{(t)}, \quad \Expect[\bg_i^{(t)}|\btheta_t] = \nabla f(\btheta_t), \quad t \geq 0.
  \label{eq:sgd}
  \tag{SGD}
\end{align}
where $\{\gamma_t \}_{t \geq 0}$ is a step-size schedule. Implicit here is the assumption that the communication link between the clients and the server is noiseless, which we expound upon next.

{\bf Z-SGD.} In the presence of noise in the communication link from the clients to the server, the \ref{eq:sgd} algorithm modifies to
\begin{align}
\btheta_{t+1} = \btheta_t - \gamma_t \, \awgn(\{\bg_i^{(t)} \} ),
    \tag{Z-SGD}
    \label{eq:awgn_sgd}
\end{align}
where $\awgn(\cdot)$ models the noisy communication of gradients. Note that the Z-SGD has two sources of stochasticity: one stemming from the stochastic gradients and the other from the  transformation $\awgn$. %% While the gradient used in the Z-SGD update still has the same conditional mean as the noiseless case  (zero mean Gaussian in ~\ref{eq:awgn_final}), it has higher variance due to the Gaussian term. When $P = \infty$, \ref{eq:awgn_sgd} reduces to \ref{eq:sgd}. 

\iffalse 
{\bf Communication model.} To model the communication link from the clients to the server $\awgn$ in~\eqref{eq:awgn_sgd}, we consider the additive noise (AN) channels. The defining property of this family is the superposition of incoming wireless signals (enabling over-the-air computation) possibly corrupted together with an independent channel noise \cite{shi2020communication}. This class comprises some of the well-studied practical channels including the classical multiple-access-channel \cite{nazer2007computation}. We denote the channel as a (random) mapping $\awgn_P(\cdot)$, that transforms the set of messages transmitted by the clients $\{\bx_i \}_{ i \in [k]} \subset \reals^d $ to its noisy version $\by \in \reals^d$ received by the server:
\looseness=-1
\begin{align}
     \label{eq:normal_awgn}
    \by = \awgn_P(\setx) \define \sum_{i=1}^k \bx_i + \bZ, \quad \norm{\bx_i}^2 \leq P,
\end{align}
where the power $P >0 $ is fixed and known to everyone. The power constraint indirectly serves as a communication cost and encourages compression: if each client can transmit the same information $\bx_i$ via fewer entries, they can utilize more power per entry and hence a more faithful signal. We assume that the noise $\bZ \in \reals^d$ is independent of the channel inputs and has zero mean and unit variance per dimension. 
A key metric that captures the channel degradation quality is the signal-to-noise ratio per coordinate ($\snr$), defined as $\snr \define P/d $ (for signals of size $m\times n$, $\snr \define P/mn$). The larger it is the better the signal fidelity; $\snr = \infty$ corresponds to the ideal scenario when there is no noise. For the downlink communication from the server to the clients (broadcast channel), we assume that it's noiseless and thus the clients exactly receive what the server transmits \cite{fedoriginal17, fedefficiency16, fedoptim16}. In the rest of the paper by channel we mean the uplink channel. 

\fi 

{\bf Gradient transmission over the channel $\awgn$.} We model the communication of gradients from the clients to the server $\awgn$ in~\eqref{eq:awgn_sgd} as additive noise (AN) channels, where 
%% In the distributed optimization setting the goal is to communicate the local gradients $\bg_i \in \reals^d$ to the central server over the noisy channel in \prettyref{eq:normal_awgn}. Here we set the messages $\bx_i$ as linear scaling of gradients (given the linear channel), \ie $\bx_i = a_i \, \bg_i$ with the scalars $a_i \in \reals$ enforcing the power constraints:
\begin{align}
    \label{eq:weightedgrad_awgn}
    \awgn(\{\bg_i\})  =  \sum_{i=1}^k a \, \bg_i + \bZ, \quad \norm{a \, \bg_i}^2 \leq P.
\end{align}

where the power $P >0 $ is fixed and known to everyone. % The power constraint indirectly serves as a communication cost and encourages compression: if each client can transmit the same information $\bx_i$ via fewer entries, they can utilize more power per entry and hence a more faithful signal. 
We assume that the noise $\bZ \in \reals^d$ is independent of the channel inputs and has zero mean and unit variance per dimension. 

A key metric that captures the channel degradation quality is the signal-to-noise ratio per coordinate ($\snr$), defined as $\snr \define P/d $ (for signals of size $m\times n$, $\snr \define P/mn$). The larger it is the better the signal fidelity; $\snr = \infty$ corresponds to the ideal scenario when there is no noise. For the downlink communication from the server to the clients (broadcast channel), we assume that it's noiseless and thus the clients exactly receive what the server transmits \cite{fedoriginal17, fedefficiency16, fedoptim16}. In the rest of the paper by channel we mean the uplink channel. 



Now the received signal is a weighted summation of the gradients corrupted by noise, whereas we need the sum of the gradients $\sum_i \bg_i$ (upto zero mean additive noise) for the model training. Towards this goal, a common mild technical assumption is that the gradient norms $\{ \norm{\bg_i} \}$ are known at the receiver at each communication round
\cite{chang2020mac, guo2020analog} (can be relaxed in practice, \prettyref{sec:main_results}). The optimal scalars are then given by $a_i  =\sqrt{P}/(\max_j \norm{\bg_j}), \forall i \in [K]$, which are uniform across all the clients (\S~\ref{app:channel_transf}). 
% In other words, during each communication round the clients transmit their gradient norms to the server which then computes their maximum and broadcasts it back to them to compute $a_i$. 
Now substituting this $a_i$ in \prettyref{eq:weightedgrad_awgn} and rearranging, the effective channel can be written as
\begin{align}
    \tilde{\awgn}(\setg) \define \frac{1}{k} \sum_{i=1}^k \bg_i + \frac{\max_i \norm{\bg_i}}{k \sqrt{P}} \, \bZ.
    \tag{noisy channel}
    \label{eq:awgn_final}
\end{align}
Or equivalently, we can assume this as the actual channel model where the server receives the gradient average corrupted by a zero mean noise proportional to the gradients. Note that the noise magnitude decays in time as gradients converge to zero.
% When there is just a single worker, $k=1$, this simplifies to
% \begin{align}
%     \label{eq:awgn_single}
%     \by = \awgn_{P, \mathrm{eff}}(\bg_1) = \bg_1 + \frac{\norm{\bg_1}}{\sqrt{P}} \, \bZ.
% \end{align}
We denote $\tilde{\awgn}(\cdot)$ as simply $\awgn(\cdot)$ henceforth as these two mappings are equivalent. 

